Retrieval Augmented Structured Generation: Business Document Information Extraction As Tool Use

Business Document Information Extraction (BDIE) is the problem of transforming a blob of unstructured information (raw text, scanned documents, etc.) into a structured format that downstream systems can parse and use. It has two main tasks: Key-Information Extraction (KIE) and Line Items Recognition (LIR). In this paper, we argue that BDIE is best modeled as a Tool Use problem, where the tools are these downstream systems. We then present Retrieval Augmented Structured Generation (RASG), a novel general framework for BDIE that achieves state of the art (SOTA) results on both KIE and LIR tasks on BDIE benchmarks. The contributions of this paper are threefold: (1) We show, with ablation benchmarks, that Large Language Models (LLMs) with RASG are already competitive with or surpasses current SOTA Large Multimodal Models (LMMs) without RASG on BDIE benchmarks. (2) We propose a new metric class for Line Items Recognition, General Line Items Recognition Metric (GLIRM), that is more aligned with practical BDIE use cases compared to existing metrics, such as ANLS*, DocILE, and GriTS. (3) We provide a heuristic algorithm for backcalculating bounding boxes of predicted line items and tables without the need for vision encoders. Finally, we claim that, while LMMs might sometimes offer marginal performance benefits, LLMs + RASG is oftentimes superior given real-world applications and constraints of BDIE.

==> 2-background.tex <==
\section{Background}

Document information extraction refers to the process of automatically locating, extracting, and structuring specific information from document based sources, such as invoices or receipts. Over the years, AI has played a crucial role in revolutionizing this field. 
Early AI-based information extraction relied on procedural-based approaches to information extraction \cite{small2013informationExtraction} \cite{yang2019informationExtraction}. These systems employed hand-crafted rules including regular expression matching and conditional logic that identified patterns and keywords within documents to extract specific data points. While effective for well-defined tasks and structured documents, rule-based systems struggled with flexibility and scalability. They are labor-intensive to maintain, with the largest issue being the requirement of continuous rule updates for handling variations in language and document formats.

In more recent years, statistical approaches emerged as an alternative for document information extraction, leveraging machine learning and deep learning techniques \cite{small2013informationExtraction}. These methods involved using large annotated document and language sets which statistical models were applied to to effectively perform information extraction. The models learned to identify patterns and relationships between textual features and desired information. Techniques here included part-of-speech (POS) taggers \cite{toutanova-etal-2003-feature} which could accept textual input and output the grammatical structure of a document. Using tooling like the POS tagger, deep learning has extensively been applied to the IE problem \cite{hammerton-2003-named}. Long-Short term memory networks have been applied to IE using part of speech tagging as input.
The recent emergence of Large Language Models (LLMs) has significantly impacted the field of document information extraction \cite{perot2023lmdx}. Approaches using LLMs rely on a pipeline of performing optical character recognition to convert the document into a textual input, chunking the input, prompt generation and applying LLM-based inference to the chunked prompt in the hope that the LLM completions can decode the document. Results here have been promising, though this field of application is still new.


\subsection{Table Structure Recognition vs. Line Items Recognition}

Here, we make a distinction between the Table Structure Recognition (TSR) task and the Line Items Recognition (LIR) task. In TSR, we expect to receive a grid of cells (which may span multiple rows or columns) where the order of the columns are preserved. In LIR, the order of the columns does not matter so long as the columns are mapped to the proper, predefined column keys.

These tasks share two subtasks:

\begin{enumerate}
    \item \textbf{Cell Content Recognition}: where we want to maximize the accuracy of the text content of the cells
    \item \textbf{Cell Location Recognition}: where we want to maximize the accuracy of the absolute coordinates of the cells.
\end{enumerate}


The Grid Table Structure (GriTS) metric \cite{smock2023grits} is appropriate for TSR and can handle both subtasks, but it is too strict on the grid structure to be used for LIR.

Other proposed metrics for LIR such as ANLS* and DocILE, on the other hand, can only handle cell content recognition and does not penalize "shuffled" rows - for example, predicting a row in the middle of the table as the first row in the result \cite{peer2024anls}. This is because these metrics match predicted line items to ground truth line items using Maximum-Weight Bipartite Matching-based algorithms which do not preserve the order of the line items \cite{kuhn1955hungarian}. After, we introduce a new metric that can handle both subtasks and properly penalizes shuffled rows in the predictions.

\subsection{In-Context Learning and Retrieval Augmented Generation}

Retrieval augmented language models condition a foundation model on relevant data from a grounding corpus during generation, which can significantly improve performance \cite{ram2023incontext}. Retrieval augmented generation (RAG) is an extension of this, where a general purpose fine-tuning using a non-parametric retriever in addition to a query encoder assists a language model in question answering \cite{lewis2021retrievalaugmented}. In BDIE, there is the natural application of RAG where one retrieves similar documents by some metric to assist in information extraction.

\subsection{Tool Use and Structured Generation}

There have recently been numerous experiments run concerning the ability of foundation models to learn the usage of tools. We will refer to the ability of a foundation model's ability to teach themselves to use external tools via simple APIs as \textit{Tool Use}. One approach, such as ToolFormer \cite{schick2023toolformer}, is to finetune a foundation model to interface with APIs when responding to a prompt. Another approach is to constrain the outputs of a frozen model \textit{post-training}. Some such as Instructor \cite{liu2023instructor} impose "soft" constraints where they request the LLM to produce output following a certain schema and retry if they fail. Others such as Outlines \cite{willard2023outlines} impose harder constraints where they zero-out probabilities of invalid tokens.

\subsection{Structured Prompting}

When performing BDIE using a generative language model, structured output is essential for correctness. It is oftentimes the case that in a structured prediction problem such as named entity recognition, language models do not perform in a robustly generalized manner without explicit prompting \cite{lee2024structured}. Careful prompt engineering, as well as in-context learning, can correct issues in language model output \cite{zhang2024structure}. This has even been explored in the context of zero-shot document question answering explicitly, where layout-aware document and question structuring has been shown to improve question answering performance in zero-shot prompting environments \cite{wang2023latin}.

